Discovering Encrypted Bot and Ransomware Payloads Through Memory Inspection Without A Priori Knowledge

Malware writers frequently try to hide the activities of their agents within tunnelled traffic. Within the Kill Chain model the infection time is often measured in seconds, and if the infection is not detected and blocked, the malware agent, such as a bot, will often then set up a secret channel to communicate with its controller. In the case of ransomware the communicated payload may include the encryption key used for the infected host to register its infection. As a malware infection can spread across a network in seconds, it is often important to detect its activities on the air, in memory and at-rest. Malware increasingly uses encrypted channels for communicating with their controllers. This paper presents a new approach to discovering the cryptographic artefacts of real malware clients that use cryptographic libraries of the Microsoft Windows operating system. This enables malware secret communications to be discovered without any prior malware knowledge.

==> parking.tex <==
Ransomware is one of the most serious threats within information security, and an infection can lead to a large-scale loss of data, and also for system outages. This type of threat was highlighted in 2017 with the spread of the WannaCry malware within the NHS and which caused a large-scale outage of the infrastructure. Without a kill-switch on the malware, ransomware can often cause almost instance damage to a data infrastruture, and without a decryption key, it can be almost impossible to recover the original data. Many large organisation thus make sure there are back-ups of data, but for many smaller organisations it is often difficult to support the additional overhead of detection and backup software. While many systems now detect standard ransomware  packages within the network infrastructure, an adversary can often re-package an attack to focus on a given vulnerability and use defined  distribution methods. 
